Cost Issue in Estimation of Proportion in a Finite Population Divided Among Two Strata

The problem of estimation of the proportion of units with a given attribute in a~finite population is considered. From the population a sample is drawn due to the simple random sampling without replacement. There are limited funds for conducting survey sample. Suppose that the population is divided into two strata. The question now arises: how should sample sizes be chosen from each strata to obtain the best estimation of proportion without exceeding the budget planned. In the paper it is shown, that with the appropriate sample allocation the variance of the stratified estimator may be reduced up to 30% off of the standard, unstratified estimator.

==> cala.tex <==
0.	0.
0.01	0.68
0.02	1.34
0.03	1.99
0.04	2.63
0.05	3.25
0.06	3.86
0.07	4.45
0.08	5.04
0.09	5.6000000000000005
0.1	6.16
0.11	6.7
0.12	7.23
0.13	7.74
0.14	8.24
0.15	8.72
0.16	9.200000000000001
0.17	9.65
0.18	10.1
0.19	10.53
0.2	10.950000000000001
0.21	11.35
0.22	11.74
0.23	12.120000000000001
0.24	12.48
0.25	12.83
0.26	13.16
0.27	13.49
0.28	13.790000000000001
0.29	14.09
0.3	14.370000000000001
0.31	14.64
0.32	14.89
0.33	15.13
0.34	15.35
0.35000000000000003	15.57
0.36	15.76
0.37	15.950000000000001
0.38	16.12
0.39	16.28
0.4	16.42
0.41000000000000003	16.55
0.42	16.67
0.43	16.77
0.44	16.86
0.45	16.93
0.46	17.
0.47000000000000003	17.04
0.48	17.080000000000002
0.49	17.1
0.5	17.11
0.51	17.1
0.52	17.080000000000002
0.53	17.04
0.54	17.
0.55	16.93
0.56	16.86
0.5700000000000001	16.77
0.58	16.67
0.59	16.55
0.6	16.42
0.61	16.28
0.62	16.12
0.63	15.950000000000001
0.64	15.76
0.65	15.57
0.66	15.35
0.67	15.13
0.68	14.89
0.6900000000000001	14.64
0.7000000000000001	14.370000000000001
0.71	14.09
0.72	13.790000000000001
0.73	13.49
0.74	13.16
0.75	12.83
0.76	12.48
0.77	12.120000000000001
0.78	11.74
0.79	11.35
0.8	10.950000000000001
0.81	10.53
0.8200000000000001	10.1
0.8300000000000001	9.65
0.84	9.200000000000001
0.85	8.72
0.86	8.24
0.87	7.74
0.88	7.23
0.89	6.7
0.9	6.16
0.91	5.6000000000000005
0.92	5.04
0.93	4.45
0.9400000000000001	3.86
0.9500000000000001	3.25
0.96	2.63
0.97	1.99
0.98	1.34
0.99	0.68
1.	0.

==> calaw50.tex <==
0.	0.
0.01	0.91
0.02	1.8
0.03	2.67
0.04	3.5300000000000002
0.05	4.36
0.06	5.18
0.07	5.98
0.08	6.76
0.09	7.5200000000000005
0.1	8.27
0.11	8.99
0.12	9.700000000000001
0.13	10.39
0.14	11.06
0.15	11.71
0.16	12.34
0.17	12.96
0.18	13.56
0.19	14.14
0.2	14.700000000000001
0.21	15.24
0.22	15.76
0.23	16.27
0.24	16.75
0.25	17.22
0.26	17.67
0.27	18.1
0.28	18.52
0.29	18.91
0.3	19.29
0.31	19.650000000000002
0.32	19.990000000000002
0.33	20.31
0.34	20.61
0.35000000000000003	20.900000000000002
0.36	21.16
0.37	21.41
0.38	21.64
0.39	21.85
0.4	22.04
0.41000000000000003	22.22
0.42	22.38
0.43	22.51
0.44	22.63
0.45	22.73
0.46	22.82
0.47000000000000003	22.88
0.48	22.93
0.49	22.95
0.5	22.96
0.51	22.95
0.52	22.93
0.53	22.88
0.54	22.82
0.55	22.73
0.56	22.63
0.5700000000000001	22.51
0.58	22.38
0.59	22.22
0.6	22.04
0.61	21.85
0.62	21.64
0.63	21.41
0.64	21.16
0.65	20.900000000000002
0.66	20.61
0.67	20.31
0.68	19.990000000000002
0.6900000000000001	19.650000000000002
0.7000000000000001	19.29
0.71	18.91
0.72	18.52
0.73	18.1
0.74	17.67
0.75	17.22
0.76	16.75
0.77	16.27
0.78	15.76
0.79	15.24
0.8	14.700000000000001
0.81	14.14
0.8200000000000001	13.56
0.8300000000000001	12.96
0.84	12.34
0.85	11.71
0.86	11.06
0.87	10.39
0.88	9.700000000000001
0.89	8.99
0.9	8.27
0.91	7.5200000000000005
0.92	6.76
0.93	5.98
0.9400000000000001	5.18
0.9500000000000001	4.36
0.96	3.5300000000000002
0.97	2.67
0.98	1.8
0.99	0.91
1.	0.

==> n1-180.tex <==
0.	0
0.01	0.68
0.02	1.33
0.03	1.96
0.04	2.56
0.05	3.13
0.06	3.68
0.07	4.21
0.08	4.7
0.09	5.18
0.1	5.62
0.11	6.04
0.12	6.44
0.13	6.8
0.14	7.15
0.15	7.46
0.16	7.75
0.17	8.02
0.18	8.26
0.19	8.47
0.2	8.66
0.21	8.82
0.22	8.950000000000001
0.23	9.06
0.24	9.15
0.25	9.21
0.26	9.61
0.27	10.
0.28	10.370000000000001
0.29	10.73
0.3	11.07
0.31	11.39
0.32	11.700000000000001
0.33	11.99
0.34	12.26
0.35000000000000003	12.52
0.36	12.75
0.37	12.98
0.38	13.19
0.39	13.38
0.4	13.55
0.41000000000000003	13.71
0.42	13.85
0.43	13.97
0.44	14.08
0.45	14.17
0.46	14.24
0.47000000000000003	14.3
0.48	14.34
0.49	14.370000000000001
0.5	14.38
0.51	14.370000000000001
0.52	14.34
0.53	14.3
0.54	14.24
0.55	14.17
0.56	14.08
0.5700000000000001	13.97
0.58	13.85
0.59	13.71
0.6	13.55
0.61	13.38
0.62	13.19
0.63	12.98
0.64	12.75
0.65	12.52
0.66	12.26
0.67	11.99
0.68	11.700000000000001
0.6900000000000001	11.39
0.7000000000000001	11.07
0.71	10.73
0.72	10.370000000000001
0.73	10.
0.74	9.61
0.75	9.21
0.76	9.15
0.77	9.06
0.78	8.950000000000001
0.79	8.82
0.8	8.66
0.81	8.47
0.8200000000000001	8.26
0.8300000000000001	8.02
0.84	7.75
0.85	7.46
0.86	7.15
0.87	6.8
0.88	6.44
0.89	6.04
0.9	5.62
0.91	5.18
0.92	4.7
0.93	4.21
0.9400000000000001	3.68
0.9500000000000001	3.13
0.96	2.56
0.97	1.96
0.98	1.33
0.99	0.68
1.	0.

==> n1-438.tex <==
0.	    0
0.01	0.84
0.02	1.67
0.03	2.46
0.04	3.24
0.05	3.99
0.06	4.72
0.07	5.43
0.08	6.12
0.09	6.78
0.1	    7.42
0.11	8.03
0.12	8.63
0.13	9.20
0.14	9.74
0.15	10.27
0.16	10.77
0.17	11.25
0.18	11.71
0.19	12.14
0.2	    12.55
0.21	12.94
0.22	13.3
0.23	13.65
0.24	13.97
0.25	14.26
0.26	14.54
0.27	14.79
0.28	15.02
0.29	15.22
0.3	    15.4
0.31	15.56
0.32	15.70
0.33	15.81
0.34	15.91
0.35	15.97
0.36	16.02
0.37	16.04
0.38	16.04
0.39	16.02
0.4	    15.97
0.41	15.91
0.42	15.81
0.43	15.700000000000001
0.44	15.56
0.45	15.4
0.46	15.22
0.47	15.01
0.48	14.79000
0.49	14.540000000000001
0.5	    14.26
0.51	14.540000000000001
0.52	14.79000
0.53	15.01
0.54	15.22
0.55	15.4
0.56	15.56
0.57	15.7001
0.58	15.81
0.59	15.91
0.6	15.97
0.61	16.02
0.62	16.04
0.63	16.04
0.64	16.02
0.65	15.97
0.66	15.91
0.67	15.81
0.68	15.700000000000001
0.6900000000000001	15.56
0.7000000000000001	15.4
0.71	15.22
0.72	15.02
0.73	14.790000000000001
0.74	14.540000000000001
0.75	14.26
0.76	13.97
0.77	13.65
0.78	13.3
0.79	12.94
0.8	12.55
0.81	12.14
0.8200000000000001	11.71
0.8300000000000001	11.25
0.84	10.77
0.85	10.27
0.86	9.74
0.87	9.200
0.88	8.63
0.89	8.03
0.9	    7.42
0.91	6.78
0.92	6.12
0.93	5.43
0.94	4.72
0.950	3.99
0.96	3.24
0.97	2.46
0.98	1.67
0.99	0.84
1.	0. 
